APPTeK: Agent-Based Predicate Prediction in Temporal Knowledge Graphs

In temporal Knowledge Graphs (tKGs), the temporal dimension is attached to facts in a knowledge base resulting in quadruples between entities such as (Nintendo, released, Super Mario, Sep-13-1985), where the predicate holds within a time interval or at a timestamp. We propose a reinforcement learning agent gathering temporal relevant information about the query entities' neighborhoods, simultaneously. We refer to the encodings of the explored graph structures as fingerprints which are used as input to a Q-network. Our agent decides sequentially which relation type needs to be explored next to expand the local subgraphs of the query entities. Our evaluation shows that the proposed method yields competitive results compared to state-of-the-art embedding algorithms for tKGs, and we additionally gain information about the relevant structures between subjects and objects.

==> _mira.tex <==
\section{MIRA - tKGR Agent}
\label{sec:mira}
\iffalse
In this section, we give a formal problem definition of relation prediction in \ref{sec:problem_definition}. The procedure of how the agent gathers and processes information is presented in \ref{sec:mdp}, and the computation of Q-values is presented in detail in section \ref{sec:model_architecture}.
\fi

%%% SECTION PRELIMINARIES
\input{_problemDefinition}
%%%

\subsection{MDP Formulation}
\label{sec:mdp}
The goal of our tKGR agent is learning to reason based on the known quadruples within the tKG. Specifically, given the source entity $s$, the target entity $o$, and the temporal information $t$, the agent extends the set of known facts by selecting relation types being adjacent to any of the known entities. The set of observed facts within both topologies acts as evidence for the prediction and offers an explanation for the predicted relation. Thus, the agent learns to build topologies containing relevant information for describing the relation between $s$ and $o$ at time $t$. For the sake of brevity, we will use $x$ to substitute $\{s,o\}$ but underline that the agent operates always on both topologies, simultaneously. 

First, we provide the definition of a Markov Decision Process (MDP) and how it applies to our setting. An MDP is defined by the tuple $(S, A, R, P)$, where $S$ is the set of states, $A$ is the set of actions, $R$ is the reward function and $P$ is the state transition probability. 

\subsubsection{Action Space $A$}\hfill\\
\label{subsec:action_space}
The agent selects an action $a^i$ at iteration $i$. We define the agent's possible action space as the union of all relational types being adjacent to the topology of either the subject $s$ or the object $o$.

In order to prevent the agent to re-select relations, we distinguish between sets of relations that have already been taken into account %by the agent 
and relations that can be explored in succeeding steps. Therefore, we introduce the core information $c_x^i$ %in the $i$-th iteration 
and the periphery information $p_x^i$ of a topology, starting from the query entities $x\in \{s,o\}$.

\noindent\textbf{Core Information. } The core information stores information about the relations with their respective temporal information having been considered by the agent in the past. Hence, it encodes the history of all traversed links. Initially, it is the empty set. In each step, it is extended by relations with their timestamps matching the agent's selected relational type. We define:
\begin{equation}
    \label{eq:core}
    c_x^i \coloneqq \left\{c_{x}^{i-1} \cup r^{i}\right\}  \quad c_x^0 \coloneqq \varnothing
%    c_s^i \coloneqq \left\{c_{s}^{i-1} \cup r^{i}\right\}  \quad c_s^0 \coloneqq \varnothing
%    \qquad
%    c_o^i \coloneqq \left\{c_{o}^{i-1} \cup r^{i}\right\}  \quad c_o^0 \coloneqq \varnothing
\end{equation}
where $r^i$ denotes the set of \emph{(relation, timestamp)}-pairs, for which the relational type %of added relations 
matches the agent's chosen action $a^i$.

\noindent\textbf{Periphery Information. } The periphery information is used to define the agent's possible action space. In each step, it includes the specific first order proximity information of the entities within the observed topologies.
Initially, the both periphery sets consist of relations being incident to the query entities $s$ and $o$. After the agent's action, the periphery information is extended by relations being incident to any entities which are reachable by the information stored in the core of the topology. We define the periphery information starting from $x\in \{s,o\}$ at iteration $i$ as follows:
\begin{equation}
    \label{eq:periphery}
    p_x^i \coloneqq \{\bigcup_{v \in N_u(a^i)} N(v) \} \cup (p_x^{i-1}\setminus r^{i}) \qquad p_x^0 \coloneqq \{N(x)\},
\end{equation}
% \begin{equation}
%     \label{eq:periphery}
%     p_x^i \coloneqq \left\{\{\bigcup_{v \in N_u(a^i)} N(v) \} \cup p_x^{i-1}\right\} \setminus r^{i} \qquad p_x^0 \coloneqq \{N(x)\},
% \end{equation}

where $N_u(a^i)$ have the form $(u, a^i, v, t) \subseteq \text{Core}^i$ with $Core^i$ referring to the quadruples being reachable in the core of a topology, and $N(v)$ defines the relational neighborhood of entity $v$, i.e., \emph{(relation, timestamp)}-pairs incident to $v$, that are not covered by the core.

The proposed agent follows links not solely starting at one particular entity, which would result in linear inference paths. Instead, our agent adds all adjacent links of the selected relation type at once to gather information helping in succeeding inference steps. Consequently, we define the set of feasible actions at iteration $i$ as the relational types $r(\cdot)$ included in the union of the periphery information of the topologies starting from $s$ and $o$: $A^i \coloneqq r(p_s^i \cup p_o^i)$ where $r(\cdot)$ extracts the relational types of the \emph{(relation, timestamp)}-pairs.
%$\mathcal{A}^i \overset{\triangle}{=} \bigcup_{k=0}^i \mathcal{E}_{n_i} \cup \{STOP\}$.

%\begin{example}
%Considering the agent's graph exploration in figure \ref{fig:fingerprint} which illustrates the three steps with $tkNN=2$. For a concise representation we show the exploration only for one entity of a query quadruple $x\in {s,o}$. Starting from $x$, the agent gathers incident relations fullfilling the temporal proximity. Red crosses illustrate relations which are incident to one of the entities within the topology but can be pruned as they are not in the set of the temporal nearest neighbors. The lighter areas highlight the periphery information, whereas darker areas highlight the core information. The agent's actions are illustrated with green. In each step, the agent expands the topology around the query entity $x$ by relations fulfilling both conditions. 
%\end{example}
  
  
\begin{figure*}
    \resizebox{\textwidth}{!}{
        \input{tikz_graphfingerprint_2}
    }
    \caption{\small Left: Example of i=1,2,3 steps gathering information about the subject/object entity ($x \in \{s,o\}$). Brighter areas highlight the periphery information $p_x^i$; darker areas highlight the core information $c_x^i$. Red crosses illustrate paths being pruned due to the temporal proximity constrain $tknn=2$; Right: Computation of the graph fingerprint $\Phi_x$; input to the MLP constructed by concatenating the embeddings for the relations $\psi(p) $with their respective temporal embeddings $\xi(t)$ in $c_x$ and $p_x$}
    \label{fig:fingerprint}
\end{figure*}


%
% SEC: STATE SPACE
%
\subsubsection{State Space $S$}\hfill\\
For the description of the state space, we have to consider two aspects. Each succeeding quadruple the agent chooses is \emph{i)} incident to the inferred set of the explored topology; \emph{ii)} closely related to the temporal information encoded within the query. 

\textbf{i)} Incident relation\hfill\\
We define the state $s_x^{i}$ of topologies starting from $x\in \{s,o\}$ at iteration $i$ by joining the core (eq. \ref{eq:core}) and periphery (eq. \ref{eq:periphery}) information:
\begin{equation}
    % s_{s}^{i} \coloneqq c_{s}^{i} \cup p_s^{i} \quad s_{s}^{0} \coloneqq \{N(s)\}, \qquad
    % s_{o}^{i} \coloneqq c_{o}^{i} \cup p_o^{i} \quad s_{o}^{0} \coloneqq \{N(o)\},
    s_{x}^{i} \coloneqq c_{x}^{i} \cup p_x^{i}% \quad %s_{x}^{0} \coloneqq \{N(x)\},
\end{equation}

The state representation of the subject and object entity is calculated by a non-linear transformation function $\Phi : s_x \rightarrow \Phi(s_x)\in \mathbbm{R}^f$ being explained in more detail in section \ref{subsubsec:fingerprint}. The overall state representation combines both state representations as follows:
\begin{equation}
    s^i \coloneqq h(\Phi(s_{s}^{i}), \Phi(s_{o}^{i})).
\end{equation}
The function $h(\cdot, \cdot)$ denotes an aggregation function summarizing the observed topologies of the query entity pair, i.e., of the subject and object entity. 
As aggregation function $h$, we can choose from several alternatives:


\begin{tabular}[t]{l|p{6cm}}
     $\bullet$~Concat & $h(\Phi(s_{s}^{i}), \Phi(s_{o}^{i})) = \Phi(s_{s}^{i}) || \Phi(s_{o}^{i})$\\
     $\bullet$\makecell{Element-\\~wise max} & $h_k(\Phi(s_{s}^{i}), \Phi(s_{o}^{i})) = %\underset{1 \leq k\leq m}{\max}
     \max(\Phi_k(s_{s}^{i}),  \Phi_k(s_{o}^{i}))$\\
     $\bullet$~Sum & $h(\Phi(s_{s}^{i}), \Phi(s_{o}^{i})) = \Phi(s_{s}^{i}) \oplus \Phi(s_{o}^{i})$ \\
     $\bullet$~Hadamard & $h(\Phi(s_{s}^{i}), \Phi(s_{o}^{i})) = \Phi(s_{s}^{i}) \odot \Phi(s_{o}^{i})$
\end{tabular}
% \begin{itemize}
% %\begin{description}[leftmargin=6em,style=nextline, font=\normalfont\itshape]
%     \item [Concat.] \qquad~\qquad $h(\Phi(s_{s}^{i}), \Phi(s_{o}^{i})) = \Phi(s_{s}^{i}) || \Phi(s_{o}^{i})$
%     \item[\shortstack{Element-\\wise Max.}] 
%     $h_k(\Phi(s_{s}^{i}), \Phi(s_{o}^{i})) = \underset{1 \leq k\leq m}{\max}(\Phi(s_{s}^{i}),  \Phi(s_{o}^{i}))$
%     \item [Sum.] $h(\Phi(s_{s}^{i}), \Phi(s_{o}^{i})) = \Phi(s_{s}^{i}) \oplus \Phi(s_{o}^{i})$
%     \item [Hadamard.] $h(\Phi(s_{s}^{i}), \Phi(s_{o}^{i})) = \Phi(s_{s}^{i}) \odot \Phi(s_{o}^{i})$
% %\end{description}
% \end{itemize}
where $\Phi_k(\cdot)$ denotes the $k$-th entry of the vector representation. In the following, we will use the \emph{Concat} function as aggregation function.


\textbf{ii)} Temporal proximity\hfill\\
Additionally, we constrain the set of possible actions in the periphery by the temporal domain. The agent explores only adjacent facts that have a temporal proximity to the query quadruple. The intuition is that the agent's inference is based on quadruples which are relevant w.r.t the temporal information given in the query. Let $q_q = (s_q, p_q, o_q, t_q)$ be a query quadruple and $\mathcal{C}$ be a candidate set of incident quadruples fulfilling the first condition (i)). Then, for each quadruple $q_i = (s_i, p_i, o_i, t_i) \in \mathcal{C}$, we compute a temporal difference $\Delta t = |t_q - t_i|$. Furthermore, let $\Delta t_{kNN}$ be the $k$-th nearest neighbor distance w.r.t the temporal information. The agent's next choices of relational types is constrained by:
\begin{equation}
N_{tkNN}(q_q) = \left\{p_i | \forall (s_i, p_i, o_i, t_i) \in \mathcal{C} : \Delta t = |t_q - t_i| < \Delta t_{kNN}\right\}.
\end{equation}
In other words $\neg \exists (s_j, p_j, o_j, t_j) \notin N_{tkNN}(q_q) : \Delta t = |t_q - t_j| < \Delta t_{kNN} $. In the following, we associate adjacent relations in the periphery with this temporal filtering step being applied. % and omit the index $tkNN$. % and abbreviate $N_{tkNN}(v|t_0)$ by $N(v)$. 

\begin{example}
Fig. \ref{fig:fingerprint} shows three steps with $tkNN=2$ of the agent's graph exploration. For a concise representation, we show the exploration only for one query entity $x\in \{s,o\}$. Starting from $x$, the agent gathers incident relations (cond. i)) fulfilling the temporal proximity (cond. ii)). Red crosses indicate relations being incident to one of the entities within the topology but can be pruned as they are not in the set of the temporal nearest neighbors. For the query $q_q = (s_q, ?, o_q, t_q)$, the agent can choose amongst $|N_{tkNN}(q_q)|=2$ relations at step $1$. The lighter (darker) areas highlight the periphery (core) information.%, whereas darker areas highlight the core information. 
Initially, the core information is the empty set. The agent's actions are illustrated by green edges. In each step, the agent expands the topology around the query entity $x$ by relations fulfilling both conditions, and therefore, learns iteratively more about an entity's neighborhood.
\end{example}


\subsubsection{Transition}\hfill\\
The transition function $f: S \times r \rightarrow S$ is defined as $f(S^i, r^i) = (c_s^{i+1}, p_s^{i+1}, c_o^{i+1}, p_o^{i+1})$, correspondingly.

\subsubsection{Reward $R$}\hfill\\
\label{subsubsec:reward}
The agent is expected to learn useful motifs in the tKG only when it learns to predict the correct target linkage between the query subject and object. It receives a terminal reward of $1$ if the topologies of the subject and object overlap in at least one entity such that there exists a path connecting both entities, and $0$ otherwise. All intermediate states receive a reward of $0$.
We define the reward as: 
\begin{equation}
\label{eq:reward}
    \mathbbm{1}\{\bigcup_{(r,t) \in c_s^{i+1}} N(r) \cap \bigcup_{(r,t) \in c_o^{i+1}} N(r)\}.
\end{equation}
Generally, let $Q_\theta (s^i, a^i)$ be the Q-function where $\theta$ defines the model's parameters. The Q-function defines the long-term reward of taking action $a^i$ at state $s^i$, and following the optimal policy after that. The objective is to learn a value function approximator maximizing Q-values for correctly identifying the target relation. 

For relation prediction, given a query, the reasoning about the relational type is based on both topologies. Likewise to \cite{lao-etal-2011-random, xiong-etal-2017-deeppath}, these can be used as logical formulas to infer the relation type. In other words, the topologies are used as binary features (c.f. eq.\ref{eq:reward}) upon which a classifier is learned. In our evaluation in section \ref{subsec:relation_prediction} we use a simple linear regression layer. 

%In the next section, we introduce our model, \emph{MIRA}, which first uses a pre-processing step to learn a representation of the agent's state, and secondly, how this representation is used to compute relevant q-values.


\subsection{Model architecture}
\label{sec:model_architecture}
%Next, we introduce the architecture of MIRA in more detail. It is 
%Our model, MIRA, is divided into two modules: one module to compute a representation (fingerprint) of the observed topology%, referred to as a \emph{fingerprint}
%; and one to compute Q-values while masking out unreachable actions.

%\inlineheader{Calculating Fingerprint}
%\label{subsubsec:fingerprint}
%
% START --- BINARY ARCHITECTURE
%

%On traversing the knowledge base starting from the subject entity and object entity, the agent gathers more and more information in the $k$-th order proximity. As discussed in section \ref{sec:mdp}, the current state is defined by the topology's core information $c_x^{(i)}$ for entity $x$=\emph{subject | object} at iteration $i$ and the periphery information $p_x^{(i)}$. The computation of the fingerprint translates the herein stored relation information in two binary vectors, one $|R|$-dimensional vector for the relation type being activated, and another $|T|$-dimensional vector is used for the temporal information. Therefore, we define:
%\begin{equation}
%    \mathbbm{1}_{rel} = 
%    \begin{cases} 1 &\text{if } r_k \in p_x^{(i)} \cup c_x^{(i)}\\
%                0 &\text{otherwise}
%    \end{cases}
%\end{equation}
%\begin{equation}
%    \mathbbm{1}_{time} = 
%    \begin{cases} 1 &\text{if } \exists (s, p, o, t_k) \in p_x^{(i)} \cup c_x^{(i)}\\
%                0 &\text{otherwise}
%    \end{cases}
%\end{equation}

%After the topology's information is translated to binary vectors, we concatenate them and use them as input for a deep forward network yielding a fingerprint for the topology denoted by $\Phi_x$ where $x$ is the starting entity $s$ or $o$. In other words, the function $\Phi: U \rightarrow R^d$ describes a non-linear transformation from the space $U \subseteq \mathbbm{1}_{rel} \times \mathbbm{1}_{time}$ to a lower $d$-dimensional vector in the real vector space. 
%The fingerprints are calculated for both topologies, one starting from the head entity and the other one starting from the tail entity, i.e., we get $\Phi_h$ and $\Phi_t$.
%The architecture for computing the fingerprints are illustrated in figure \ref{fig:fingerprint}, where the red edges in the subgraph illustrates the edges in $c_x^{(i)}$ and the blue edges are the ones from the perihpery $p_x^{(i)}$.

%
% END --- BINARY ARCHITECTURE
%


\subsubsection{Calculating Fingerprint}\hfill\\
\label{subsubsec:fingerprint}
%
% MAX ARCHITECTURE
%
On traversing the tKG starting from $x \in \{s, o\}$, the agent gathers iteratively information about their respective neighborhood. As discussed in section \ref{sec:mdp}, the current state for $x$ at iteration $i$ is defined by the topology's core information $c_x^{i}$ and its periphery $p_x^{i}$. Generally, the computation of the fingerprint translates the herein stored information about the relations in a $d_f$-dimensional vector. This is accomplished by concatenating embeddings for relations, denoted by $\psi: r \rightarrow \mathbbm{R}^{d_r}$, with their corresponding embeddings of the temporal domain, denoted by $\xi: t \rightarrow \mathbbm{R}^{d_t}$. We define:
\begin{equation}
    \mathbbm{X}_{c_x^{i} \cup p_x^{i}} = \underset{(p, t) \in c_x^{i} \cup p_x^{i} }{\parallel_0} (\psi(p)\parallel_1 \xi(t)),
\end{equation}
where $\parallel_l$ denotes the concatenation in the $l$-th dimension. %Therefore, 
The input to the MLP is a $|c_x^{i} \cup p_x^{i}| \times (d_r + d_t)$ dimensional matrix denoted by $\mathbbm{X}_{c_x^{i} \cup p_x^{i}}$, where $d_r$ denotes the dimension of the embedding of the relations, and $d_t$ the one of the temporal embeddings. The network's output yields a $|c_x^{i} \cup p_x^{i}| \times d_f$ dimensional vector. Finally, a max-pooling operation of the $0$-th dimension yields the $d_f$-dimensional fingerprint. We denote this transformation by $\Phi_x$.

%The fingerprints are calculated for both topologies %starting from $s_q$ and $o_q$ of a query, i.e., we compute
%yielding $\Phi_s$ and $\Phi_o$. 
The calculation of a fingerprint is illustrated in fig. \ref{fig:fingerprint} (right). The core's information of the topology (green) is concatenated with the relational information given in the periphery (red). The input to the MLP is shown with the concatenation of the relation embeddings with their respective temporal embeddings. After a softmax operation, the network yields a fingerprint $\Phi_x$ of the observed topology.

\subsubsection{Q-network}\hfill\\
The RL frameworks in \cite{xiong-etal-2017-deeppath, das-2017-minerva, lin-2018-multihop, Shen2018MWalkLT} have to handle large action spaces, which leads to problems when we lack of some actions for training labels. In the worst case, there could be no samples for certain relations that lead to random outputs. Therefore, each of the earlier works proposed workarounds either by defining a more sophisticated reward function \cite{xiong-etal-2017-deeppath, lin-2018-multihop} or by combining the learning procedure with MCTS \cite{Shen2018MWalkLT}, which tackles the sparse reward setting. In our approach, we use a DQN with action masking for relations having been identified in the filtering step described in section \ref{subsec:action_space}.

Having computed the fingerprints %(c.f. sec \ref{subsubsec:fingerprint}) 
for both topologies, we concatenate them $\Phi_s || \Phi_o$ and get a $(2 \cdot d_f)$-dimensional input vector for the Q-net. 
Thereafter, we compute the Q-values for all relational types. An MLP is used as function approximator $\hat{q}_{\theta} = \hat{q}_{\theta} (s, a; \theta)$. %where $\theta$ denotes the network's parameters 
%(c.f. section \ref{subsubsec:deepqlearning}).

Next, we discuss the shrinkage of the agent's search space amongst the possible actions at iteration $i$ by applying action masking. As a large action space might lead to poor convergence, we use this additional masking to disguise all relational types being not reachable in the agent's current state, i.e., there are types of relations that are not incident to any entity in any of the two observed topologies and that are not in temporal proximity to the query quadruple. Therefore, they are not relevant for the agent's next choice. %(c.f. \ref{subsec:action_space}). 
Recall that the agent's possible relations for further exploration are stored within a topology's periphery $p_x^{(i)}$. We use this information to cloak all unreachable semantic links by defining a binary mask $\Omega^i \in \{0,1\}^{|\mathcal{R}|}$ that retains only the information of traversable relations in the agent's current state. Formally, it is defined as:
\begin{equation}
    \Omega^{(i)}(r_k) = 
    \begin{cases} 1 &\text{if } r_k \in r(p_s^{(i)} \cup p_o^{(i)})\\
                0 &\text{otherwise}.
    \end{cases}
\end{equation}
The network's outputs for all relations is defined by $f (s^i, \theta) \rightarrow [\hat{q}(s^i, a_0), \hat{q}(s^i, a_1), \ldots, \hat{q}(s^i, a_n)]$, where $f(s^i, \theta)$ describes the non-linear transformation of state $s^i$ in the $i$-th iteration. %of the learning procedure. 
We apply the \emph{Hadamard} product for masking. We compute:%to mask out all unreachable relations. Therefore, we compute:
\begin{equation}
    f_{\Omega^i}(s^i, \theta) = [\hat{q}(s^i, a_0), \hat{q}(s^i, a_1), \ldots, \hat{q}(s^i, a_n)] \odot \Omega^i,
\end{equation} 
yielding only relevant Q-values which the agent has to take into consideration. The architecture is illustrated in figure \ref{fig:qnet} where two relational types are masked out in the final output.

%
% SECTION : DEEP Q Learning
%
\subsubsection{Deep Q-Learning - Learning Procedure}\hfill\\
\label{subsubsec:deepqlearning}
In deep Q-learning, we apply a function approximator $\hat{q}_{\theta} = \hat{q}_{\theta} (s, a; \theta)$, where $\theta$ are the model's parameters. The objective function being optimized is straightforward defined as:
\begin{equation}
\mathcal{L}(\theta) = \mathbbm{E}\left[ \left(r(s_t, a_t) + \gamma \max_a \hat{q}_\theta (s_{t+1},a) - \hat{q}_\theta (s_t, a_t) \right)^2 \right]
\end{equation}

For an effective learning procedure, it has been shown by \cite{mnih2013atari}, that using a \emph{Replay Memory} is of discernible utility. Hence, we store the transitions $(s_t, a_t, r_t, s_{t+1})$ in $\mathcal{D}$, and a batch is defined by a sample taken from the replay memory, $(s_j, a_j, r_j, s_{j+1})\sim \mathcal{D}$. 
%It is generally known that 
Generally, it is beneficial to learn from the same transitions multiple times which greatly facilitates a stable learning process.
%It is generally known, the benefit lies in the fact that this allows for learning from the same transition multiple times and greatly improves a stable learning process.

\begin{figure}
    \centering
    \resizebox{0.65\linewidth}{!}{
        \input{tikz_dqn}
    }
%    \caption{Q-Net of MIRA where an action masking is applied on the last layer}
    \caption{MIRA's Q-Net with action masking on last layer}
    \label{fig:qnet}
\end{figure}

==> _qLearning.tex <==
% !!!!!


%  ####   DONT DELETE    #### 


% !!!!!

\subsection{Q-Learning}
\textcolor{cyan}{revise - shorten chapter 4.2}

In Q-learning we want to explore all possibilities of state-action pairs in order to get an estimation of the long-term reward the agent will receive by applying a specific action in a state. 
Generally, a positive reward leads to the agent's tendency to choose this action in a similar state next time such that we can derive a best guess at an optimal policy from action values $Q(s,a)$, we can typically calculate as: 
\begin{equation}
    \pi(s) = \argmax_a Q(s,a)
\end{equation}
The reinforcement learning frameworks defined in \cite{xiong-etal-2017-deeppath, das-2017-minerva, lin-2018-multihop, Shen2018MWalkLT} have to handle a large action space which lead to problems when we lack of some actions for training labels. In the extreme case, there could be no examples for certain relations which lead to a random output of the corresponding. Each of the earlier works therefore proposed workarounds either by defining a more sophisticated reward function \cite{xiong-etal-2017-deeppath, lin-2018-multihop} or by combining the learning with MCTS \cite{Shen2018MWalkLT} which tackles the sparse reward setting. 

\inlineheader{Deep Q-Learning}
%\subsubsection{\bfseries Deep Q Learning}\hfill\\
\label{subsubsec:deepqlearning}
To handle very large state space, in deep q learning we introduce a function approximator $\hat{q}_{\theta} = \hat{q}_{\theta} (s, a; \theta)$, where $\theta \in \mathbbm{R}^M$ is a vector that parametrizes the function approximator. These parameters are the weights in a neural network architecture. This is used in the Deep Q Learning algorithm which otherwise is similar to Q-learning, where we at time $t$ use the TD-target $r(s_,a_t) + \gamma \max_a \hat{q}_\theta(s_{t+1}, a)$. To improve the approximation $\hat{q}_\theta$ we define a Loss function $\mathcal{L}(\theta)$ and attempt to minimize it,
\begin{equation}
    \mathcal{L}(\theta) = \mathbbm{E}\left[ \left(r(s_t, a_t) + \gamma \max_a \hat{q}_\theta (s_{t+1},a) - \hat{q}_\theta (s_t, a_t) \right)^2 \right]
\end{equation}
The minimization is done by taking the semi-gradient of $\mathcal{L}(\theta)$ with respect to $\theta$. That is, 
\begin{equation}
\resizebox{\columnwidth}{!}{
$    \nabla_{\theta} \mathcal{L}(\theta) = \mathbbm{E}\left[ 2 \left(r + \gamma \max_a \hat{q}_{\theta} (s_{t+1}, a) - \hat{q}_{\theta} (s_t, a_t) \nabla_\theta \hat{q}_\theta (s_t, a_t)  \right) \right]$
}
\end{equation}
Estimating the expected value can be computationally demanding, the mean of $r +\gamma \max_a \hat{q}_\theta (s_{t+1}, a) - \hat{q}_\theta (s_t, a_t) \nabla_\theta \hat{q}_\theta (s_t, a_t)$ has to be calculated for every accessible state-action pair. It is often more favorable to optimize the loss function using stochastic gradient descent (SGD). Optimizing the loss function is then done using the gradient above without the expected value.

To avoid the correlation and biases between samples when executing the SGD on consecutive frames, we apply a \emph{Replay Memory} \cite{mnih2013atari}, i.e., we store the transition $(s_t, a_t, r_t, s_{t+1})$ in $\mathcal{D}$, and the SGD is carried out using subsets (Batches) of the replay memory, $(s_j, a_j, r_j, s_{j+1})\sim \mathcal{D}$. This also allows for learning from the same transition multiple times.

%By using the state $s_{t+1}$ as our prediction at $s_t$, we introduce a bias in our trajectory towards $q_\ast$. We also have a strong correlation between the samples if we perform the SGD on consecutive frames. To avoid these correlations, we introduce a concept formulated in (cite; Mnih; Playing atari with deep rl) as \emph{Replay Memory} $\mathcal{D}$. The transition $(s_t, a_t, r_t, s_{t+1})$ ar estored in $\mathcal{D}$, and the SGD is carried out using subsets (Batches) of the replay memory, $(s_j, a_j, r_j, s_{j+1})\sim \mathcal{D}$. This breaks the correlation and biases, reducing oscillations and other unwanted behavior in the SGD. Replay memory also enables the agent to learn from the same transition multiple times - leading to greater data efficiency.

In order for SGD to converge, the target must be fixed. Using temporal difference: the target in the equation above depends on the parameters that we are updating at every SGD step. We thus have a moving target, which more or less ensures that the SGD will not converge. The solution to this is to compute the TD-targets with respect to fixed parameters $\Theta$. These are then updated to the current parameters $\theta$ after a specified number $C$ of learning steps. This yields a periodically stationary target for the SGD, being the standard for deep Q-nets:
\begin{equation}
\resizebox{\columnwidth}{!}{
$    \nabla_\theta \mathcal{L} (\theta) = 2 \left( r+ \gamma \max_a \hat{q}_\Theta (s_{t+1}, a) - \hat{q}_\theta (s_t, a_t) \right) \nabla_\theta \hat{q}_{\theta} (s_t, a_t)$.
}
\end{equation}



==> _table_notation_mira.tex <==
--- NOTATION TABLE ----
\newcolumntype{b}{X}
\newcolumntype{s}{>{\hsize=.2\hsize}X}

\begin{table}
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabularx}{\columnwidth}{$s|^b}
\toprule
\rowstyle{\bfseries}%
Symbol & Description\\
\midrule
$s, o$ & \textbf{s}ubject entity, \textbf{o}bject entity \\
$p$   & relation type (\textbf{p}redicate)\\
$t$ & \textbf{t}emporal information\\
$N_u(p)$ & adjacent nodes to entity $u$ by following rel. type $p$\\
$N(v)$ & adjacent relations of entity $v$\\
%$\mathcal{P}_{s \rightarrow o}$ & path set from subject ($s$) to object ($o$)\\
$c_s^{i}, c_o^{i}$ & topology's core info. of $s$, $o$ at iteration $i$\\
$p_s^{i}, p_o^{i}$ & topology's periphery info. of $s$, $o$ at it. $i$\\
$s_s^{i}, s_o^{i}$ & topology state representation of $s$, $o$ at it. $i$\\
\bottomrule
\end{tabularx}
}
\caption{Notation}
\label{tab:notation}
\end{table}


==> _table_relatedwork_rl_on_kg.tex <==
\noindent
\begin{table}[t]
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{$l^l^l^l^l}
\cmidrule{1-5}
\rowstyle{\bfseries}%
Method & State $s_t$ & Action $a_t$ & Reward $\gamma$ & Policy Network \\
\cmidrule{1-5}
%
\multicolumn{5}{l}{\cellcolor{gray!10}RL on {\bfseries static knowledge bases} for {\bfseries entity prediction} (query answering)}  \\
%
\cmidrule{1-5}
DeepPath \cite{xiong-etal-2017-deeppath} & $(e_t, e_q - e_t)$ & $\{r\}$ & $\mathbbm{1}\{e_t = e_q\}$ & FCN\\
%
MINERVA \cite{das-2017-minerva} & $(e_t, e_s, r_q, e_q)$ & $\{(e_t, r, v)\}$ & $\mathbbm{1}\{e_t = e_q\}$ & $h_t = LSTM(h_{t-1}, [a_{t-1}; o_t])$ \\
%
Multi-Hop \cite{lin-2018-multihop} & $(e_t, (e_s, r_q))$ & $\{(r', e') |(e_t, r', e') \in \mathcal{G}\}$ & $R_b(s_T) + (1-R_b(s_T)) f (e_s, r_q, e_T)$ & $h_t = LSTM(h_{t-1}, a_{t-1})$\\
%
M-Walk \cite{Shen2018MWalkLT} & $s_{t-1} \cup \{a_{t-1}, v_t, \mathcal{E}_{\mathcal{G}_{v_t}}, \mathcal{V}_{v_t} \}$ & $ \mathcal{E}_{\mathcal{G}_{v_t}} \cup \{STOP\}$ & $\mathbbm{1}\{e_t = e_q\}$ & GRU-RNN + FCN\\
%
CPL \cite{fu-2019-collaborative} Reasoner & $(e_s, r_q, h_t)$ & $\{\xi \in \mathcal{E}_{\mathcal{G}}\}$ & $\mathbbm{1}\{e_t = e_q\}$ & $h_t = LSTM(h_{t-1}, [r_{t}; e_t])$ \\
CPL \cite{fu-2019-collaborative} Extractor & $(b_{e_t}, e_t)$ & $\{(r', e')\}_{(e_t, r', e')} \in b_{e_t}$ & delayed from reasoner & PCNN-Att \\
%
%\cmidrule{1-5}
%\multicolumn{5}{l}{\cellcolor{gray!10}RL on {\bfseries static knowledge bases} for {\bfseries predicate prediction} (relation reasoning)} \\
\cmidrule{1-5}
%
%
\cmidrule{1-5}
\multicolumn{5}{l}{\cellcolor{gray!10}RL on {\bfseries non-static knowledge bases} for {\bfseries entity prediction} (query answering)}\\
\cmidrule{1-5}
%
TiTer \cite{sun-2021-timetraveler} & $s_l=(e_l, t_l, e_q, t_q, r_q)$ &
\makecell{$\{(r',e', t')|(e_l, r', e', t') \in \mathcal{F},$ \\ $ t' \leq t_l, t' \leq t_q\}$} & $R(s_L)=\mathbbm{1}(e_L = e_{gt})$ & $h_l = LSTM(h_{l-1}, [r_{r-1}; e_{l-1}^{t_{l-1}}])$ \\
TPath \cite{bai-2021-tpath} 
& $s = (e_t, e_s, r, e_o, tim)$ 
& $A_s = \{(r, tim|s)\}$
& $\mathbbm{1}\{e_t = e_q\}$
& $h_t = LSTM(a_{t-1}; o_t, h_{t-1})$ \\ 
\cmidrule{1-5}
\multicolumn{5}{l}{\cellcolor{gray!10}RL on {\bfseries non-static knowledge bases} for {\bfseries predicate prediction} (relation reasoning)}\\
\cmidrule{1-5}
%
\textbf{APPTeK} 
& $s^i \coloneqq h(\Phi(s_{s}^{i}), \Phi(s_{o}^{i}))$
& $A^i \overset{\triangle}{=} p_s^i \cup p_o^i$
& $\mathbbm{1}\left\{\bigcup_{r \in c_s^{i+1}} N(r) \cap \bigcup_{r \in c_o^{i+1}} N(r)\right\}$
& FCN with Action-masking
\end{tabular}
}
\caption{
Comparison of RL methods for reasoning on KGs;
let $e_s$ be the source entity, $e_q$ be the query entity, and $e_t$ be the entity which is explored by an agent at iteration $t$. The inference of \emph{MINERVA}, \emph{M-Walk} and \emph{CPL} use binary rewards. For the policy networks, \emph{DeepPath} uses a fully-connected network, the extractor for textual information of \emph{CPL} employs convolutional neural networks, while the rest uses recurrent neural networks. 
For MINERVA, $a_{t-1} \in \mathbb{R}^d$ and $o_t \in \mathbb{R}^d$ denote the vector representation for action/relation at time $t - 1$ and observation/entity at time $t$, respectively, and $[;]$ denotes the vector concatenation.
For Multi-Hop, $R_b(s_T)$ denotes the terminal reward, which is $1$ if the agent arrives at a correct target entity at the end of search, and $0$ otherwise. The reward function is generalized by a reward shaping strategy, where $f(e_s, r_q, e_T)$ is a pre-trained scoring function.
For CPL, $b_{e_t}$ denotes the sentence bag of the current entity. Specifically, the action space for the reasoner is defined as the union of edges in the current KG and edges extracted from a text corpus. For TiTer, $s_L$ denotes the final state at step $L$, $h_l$ denotes the representation at the $l$-th iteration}
\label{tab:scoring_fncs}
\end{table}
\noindent

==> makros.tex <==
\newcommand{\tensor}[1]{\underline{\mathcal{#1}}}
\newcommand{\actionspace}[1]{\mathcal{A}}
\newcommand{\statespace}[1]{\mathcal{S}}
